Effective Mutation Rate Adaptation through Group Elite Selection

Evolutionary algorithms are sensitive to the mutation rate (MR); no single value of this parameter works well across domains. Self-adaptive MR approaches have been proposed but they tend to be brittle: Sometimes they decay the MR to zero, thus halting evolution. To make self-adaptive MR robust, this paper introduces the Group Elite Selection of Mutation Rates (GESMR) algorithm. GESMR co-evolves a population of solutions and a population of MRs, such that each MR is assigned to a group of solutions. The resulting best mutational change in the group, instead of average mutational change, is used for MR selection during evolution, thus avoiding the vanishing MR problem. With the same number of function evaluations and with almost no overhead, GESMR converges faster and to better solutions than previous approaches on a wide range of continuous test optimization problems. GESMR also scales well to high-dimensional neuroevolution for supervised image-classification tasks and for reinforcement learning control tasks. Remarkably, GESMR produces MRs that are optimal in the long-term, as demonstrated through a comprehensive look-ahead grid search. Thus, GESMR and its theoretical and empirical analysis demonstrate how self-adaptation can be harnessed to improve performance in several applications of evolutionary computation.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> content/algo_box.tex <==
\begin{algorithm}
\captionsetup{labelfont={sc,bf}, labelsep=newline}
  \caption{The GESMR Algorithm for coevolving solutions and mutation rates using group elite selection as described in Section~\ref{sec:algorithm}.}
  \begin{algorithmic}[1]
   \STATE describe all variables, e.g. $\mathbf{\Delta} \in \mathbb{R}$
    \STATE initialize 
    $\mathbf{X}^0\in \mathbb{R}^{(N+1)\times d}$
    \STATE initialize
    $\mathbf{\sigma}^0\in \mathbb{R}^{K}$ 
    \FOR {$t=0,1,\dots, T$ } 
        \STATE $\mathbf{f}^t\in\mathbb{R}^{N+1} \gets F(X^t)$
        \STATE sort $\mathbf{X}^t, \mathbf{f}^t$ with ascending order of $\mathbf{f}^t$
        \STATE $\mathbf{X}^{t+1}_0 \gets \mathbf{X}^t_0$
        \STATE assign each $\mathbf{\sigma}^t_i$ to $N/K$ solutions from $\mathbf{X}^t$, giving $\mathbf{\sigma}^{x}\in \mathbb{R}^N$
        
        \FOR{$n=1,2,\dots, N$}
            \STATE $p \sim \text{UniformRandom}(1,N/2)$
            \STATE $\epsilon \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$
            \STATE $\mathbf{X}^{t+1}_n \gets
            \mathbf{X}^t_p + 
            \mathbf{\sigma}^x_n \epsilon $
        \ENDFOR
        
        \STATE $\mathbf{\Delta} \in \mathbb{R}^{K\times (N/K)} \gets $ 
        $N/K$ samples of function value change for all $\mathbf{\sigma}^t$
        
        \STATE $\mathbf{\delta} \in \mathbb{R}^K \gets \min_j \mathbf{\Delta}_{ij}$
        
        \STATE sort $\mathbf{\sigma}, \mathbf{\delta}$
        with ascending order of $\mathbf{\delta}$
        
        \STATE $\mathbf{\sigma}^{t+1}_0 \gets \mathbf{\sigma}^t_0$
        
        \FOR{$k=1, 2, \dots K$}
            \STATE $p \sim \text{UniformRandom}(1,K/2)$
            \STATE $\epsilon \in \mathbb{R} \sim \text{LogUniform}(2^{-1}, 2^{1})$
            \STATE 
            $\mathbf{\sigma}^{t+1}_k \gets
            \mathbf{\sigma}^t_p+\epsilon $
        \ENDFOR
    \ENDFOR
    %\STATE \textbf{Function: } evolve

    
    \label{alg:algo}
  \end{algorithmic}
\end{algorithm}


==> content/old_analysis.tex <==

\newcommand{\floor}[1]{\lfloor #1 \rfloor}
[Here I derive what the expected value of Delta is
for a Taylor series expansion of f.
I am not sure how to get the conclusion I want
from this.
The conclusion I want:
$\EX[\Delta]$ grows monotonically with 
$\sigma$ when f is "rugged".
]
\begin{align*}
    f(x)&=\sum_{q=0}^\infty \frac{f^{(q)}(a)}{q!}(x-a)^q\\
    \Delta(x,\sigma) &= f(x+\sigma\epsilon)-f(x)\\
    &=\sum_{q=1}^\infty \frac{f^{(q)}(x)}{q!}(\sigma\epsilon)^q\\
    \EX[\Delta]&=\sum_{q=1}^\infty \frac{f^{(q)}(x)}{q!}\sigma^q\EX[\epsilon^q]\\
    &=\sum_{q=1 \text{ even}}^\infty \frac{f^{(q)}(x)}{q!}\sigma^q(q-1)!!\\
    &=\sum_{q=1 \text{ even}}^\infty \frac{f^{(q)}(x)}{q!!}\sigma^q\\
\end{align*}
Assumptions:
% Gathered from:
% https://math.stackexchange.com/questions/1432419/variance-of-power-of-normal-random-variable
% https://math.stackexchange.com/questions/2245327/expected-value-of-a-non-standard-normally-distributed-variable-to-a-power#
% http://premmi.github.io/expected-value-of-minimum-two-random-variables
\begin{align*}
    &\text{for gaussian X}\\
    \EX[X^n]&=\sum_{m=0}^{\floor{n/2}} \binom{n}{2m} (2m-1)!!\sigma^{2m}\mu^{n-2m}\\
    &\text{for gaussian X with zero mean}\\
    \EX[X^n]&= (n-1)!!\sigma^{n} \text{ even n else } 0\\
    &\text{for gaussian Z with zero mean unit variance}\\
    \EX[Z^q]&=(q-1)!! \text{ even q else 0}\\
\end{align*}


%\begin{align*}
%E[X^n] &= \sigma^n (n-1)!\\
%f(x+\epsilon) - f(x) &= \frac{f'(x)}{1!}\epsilon+\frac{f''(x)}{2!}\epsilon^2+\frac{f'''(x)}{3!}\epsilon^3\\
%E[f(x+\epsilon) - f(x)] &= \frac{f'(x)}{1!}E[\epsilon]+\frac{f''(x)}{2!}E[\epsilon^2]+\frac{f'''(x)}{3!}E[\epsilon^3]\\
%E[f(x+\epsilon) - f(x)] &= \sum_{n=1}^\infty \frac{f^{(n)}(x)}{n!}E[\epsilon^n]\\
%E[f(x+\epsilon) - f(x)] &= \sum_{n=1}^\infty \frac{f^{(n)}(x)}{n!}\sigma^n (n-1)!\\
%E[\delta(x, \sigma)] &= \sum_{n=1}^\infty \frac{f^{(n)}(x)}{n}\sigma^n\\
%\end{align*}



% The problem is formulated in the 
% continuous space of $\mathbb{R}^d$
% as a minimization of the function $f(x)$
% which is continuous everywhere
% (fitness is negative of this function):
% $$\text{argmin}_{x\in \mathbb{R}^d} f(x)$$
% The genetic algorithm (GA) contains $N$ individuals,
% $x_1, \dots, x_N$ where $x_i\in \mathbb{R}^d$.
% For the sake of simplicity and to isolate the mutation operator,
% the crossover mechanism is ignored,
% and selection is done with the the 
% simplest truncation selection method. 

% \bo{you need to elaborate on what truncation selection means, and what crossover means, maybe first describe a general GA operation. Then say for the sake of simplicity, we ignore crossover, and use truncation selection method.}

% The truncation selection method
% generates the next generation's population
% by randomly selecting from the 
% best 50\% (based on function value) 
% of the current generation's population, 
% and allowing them to mutate.
% One elite is kept, which is common in GA literature
% \cite{}.
% The Gaussian mutation operator is used:
% $$M(x;\sigma) = x+\sigma \epsilon$$
% where $x$ is the solution before mutation,
% $\epsilon \sim \mathcal{N}(0,I)$ is random noise,
% and $\sigma$ is the mutation rate (MR).
% The goal of this paper is to find the optimal MR
% $\sigma_{*}$ at each generation, 
% such that the best value found by evolution
% at the end of $T$ generations (long-term) is optimized.

\label{sec:analysis}
In this section, we will analyze the local update of applying a mutation operator and provide some explanation why the vanishing MR problem exists. We leave the analysis on the long-term performance of any adaptive-MR algorithm as a future research direction.

Considering the one-step mutation operation at any particular time step $t$, we aim to find the best MR $\sigma^*$, e.g. the MR that leads to the largest performance gain. The performance gain after applying a mutation operation can be described in the following:
\begin{equation}
    \Delta(x, \sigma) = \min_{j \in [P]} f(x'_j) - f(x),~~\text{where}~~x'_j \sim M(x; \sigma).
\end{equation}
Here, $P$ is the size of the children population generated from $x$. Better $\sigma$ corresponds to lower $\Delta(x, \sigma)$. Note that $\Delta(x, \sigma)$ depends on the children population size $P$, as if we allow $P \rightarrow \infty$, clearly $\sigma^* = \infty$. The reason why we take the minimum is because the performance of the 



\textbf{When $\sigma \to 0$}:
In this case, the fitness function, $f(x)$
can be accurately estimated by a 
linear approximation using the gradient, $\nabla f(x)$:
$f(x+\sigma\epsilon) \approx f(x)+\sigma\epsilon^T\nabla f(x)$.
It follows that
$\Delta(x, \sigma) = f(x+\sigma\epsilon)-f(x) 
\approx \sigma\epsilon^T\nabla f(x)$.
Since, $\epsilon$ comes from a 
multivariate Gaussian distribution,
$\nabla f(x)$ is a non-random vector, and $\sigma$ is a scalar,
$\Delta$ comes from the zero mean Gaussian:
$$\Delta(x, \sigma) = \sigma \epsilon^T\nabla f(x) \sim 
\mathcal{N}(0, \sigma^2 \Vert \nabla f(x))\Vert^2)$$
which can be rewritten to say that
$\Delta\sim\mathcal{N}(0, v^2)$ with $v\to 0$.
This directly implies that $\EX[\Delta] = 0$
and $\EX[\min_i \Delta_i]\to 0$.

\textbf{When $0<\sigma < \sigma_c$ for small $\sigma_c$}:
$\sigma_c$ is chosen to be small enough such that
the second order and above terms disappear 
in the Taylor Expansion of $f(x)$ \akarsh{CITE THEOREM?},
leaving same linear approximation as before and that
$\Delta \sim \mathcal{N}(0, \sigma^2\Vert \nabla f(x)\Vert^2)$.
So, $\EX[\Delta]=0$ and is constant as $\sigma$ varies.
However, 
because $\min_i \Delta_i$ is a minimum of 
zero mean Gaussian random variables with finite variance,
$\EX[\min_i \Delta_i]<0$,
and $\EX[\min_i \Delta_i]$ 
monotonically decreases with larger $\sigma$ (and larger $q$) assuming $\Vert \nabla f(x)\Vert\neq 0$.
Minimizing both objectives leads to the fact that
$\sigma_*^\text{min} = \argmin_\sigma \EX[\min_i \Delta_i]$
is always greater than 
$\sigma_*^\mu = \argmin_\sigma \EX[\Delta]$.
% https://stats.stackexchange.com/questions/220/how-is-the-minimum-of-a-set-of-iid-random-variables-distributed
% https://stats.stackexchange.com/questions/226682/minimum-of-a-set-of-random-variables-that-are-normally-distributed
% https://www.untruth.org/~josh/math/normal-min.pdf
% https://stats.stackexchange.com/questions/226682/minimum-of-a-set-of-random-variables-that-are-normally-distributed

\textbf{When $\sigma \to \infty$}:
In this case,
the objective $\EX[\Delta]=\EX_x[f(x)]$ becomes no search at all,
and
the objective $\EX[\min_i\Delta_i]$ becomes random search
over the entirety of the fitness landscape.
These new solutions can both be assumed to be worse than any 
given solution, $x$, 
when we assume $x$ is at least partially optimized,
so $\EX[\Delta]>0$ and $\EX[\min_i \Delta_i]>0$.

\textbf{When $\sigma$ is moderate (Empirically)}:
At this region, it is impossible to know the distribution of
$\Delta(x,\sigma)$.
This may vary drastically depending on the specifics $f(x)$.
For example, one can imagine if $x$ is near a global maximum,
then $\EX[\Delta(x,\sigma)] \ll 0$
(vice versa for a global minimum).
This is because almost all mutations will take the solution
to a random point in the landscape definitely 
below the global maximum. 
However, a statement can still be made on this distribution
for common fitness landscapes in the common situation where
$x$ resides in a place that is
on a trajectory to a local minimum...

==> content/old_gesmr_section.tex <==

\subsection{GESMR Algorithm}
In this section, the Group Elite Selection of Mutation Rates (GESMR) is proposed to produce MRs for the $\EX[\min_i\Delta_i]$ objective from the previous section.
This method is essentially co-evolving a population
of solutions and a population of MRs in a way 
that does not decay the MRs to zero.
The detailed psuedocode for this algorithm
is in Algorithm~\ref{alg:algo}.

A population of $K$ MRs
is initialized
(usually logarithmically varying from 
$\num{1e-2}$ to $\num{1e2}$),
alongside the $N$ individual solutions
(Algorithm~\ref{alg:algo}, Line X).
At each generation, 
the population of $N$ solutions is randomly
split into $K$ groups of $N/K$ solutions
(Line X).
Each group is assigned an MR from the current
population of MRs.
The population of solutions and population of MRs
are evolved according to a simple GA
described in the problem formulation.
Each solution is evaluated using 
the functional value of the solution, $f(x)$.
Each solution is mutated according to its assigned MR.
Each MR evaluated using the \emph{best}
change in function value (over one generation)
seen in the $N/K$ samples of the MR group.
This processes involves storing mild
statistics on the change of function value
for different MRs in each generation.

==> content/trash.tex <==

GAs are known to lose population diversity without
explicit help of maintaining diversity \cite{}.
This phenomenon is natural with selection pressure \cite{}.
Because SAMR is performing selection based on the function value
$f(x_i^{(t)})$ of its pairs $(x_i^{(t)}, \sigma_i^{(t)})$,
$x_i^{(t)}$ was produced from $x_i^{(t-1)}$ using a $\sigma_i^{(t-1)}$ 
closely resembling $\sigma_i^{(t)}$,
and all $x_i^{(t-1)}$ are near each other due to the lack of a diversity preserving mechanism,
SAMR is selecting for the, on average, best mutational change
given the current population.
Essentially, over many generations, 
the pairs which consistently improves the most (a function of MR) are selected.
This translates the selection of the \textit{solutions} to the
selection of \textit{MRs} based on the MR objective $\argmin_\sigma \EX[\Delta]$ 
by noisily evaluating with a single sample of 
$\Delta(x_i^{(t-1)}, \sigma_i^{(t-1)})$.
However, because GESMR is explicitly selecting for
$\sigma$s based on the best mutation produced by that $\sigma$,
it is selecting MRs based on the MR objective $\argmin_\sigma \EX[\min_q\Delta_q]$
where $q$ becomes the group size ($N/K$).
